He Thinks He Knows Better than the Doctors: BERT for Event Factuality Fails on Pragmatics

We investigate how well BERT performs on predicting factuality in several existing English datasets, encompassing various linguistic constructions. Although BERT obtains a strong performance on most datasets, it does so by exploiting common surface patterns that correlate with certain factuality labels, and it fails on instances where pragmatic reasoning is necessary. Contrary to what the high performance suggests, we are still far from having a robust system for factuality prediction.

==> signature_expected_inf.tex <==

\paragraph{expected inf with the signatures}

Table~\ref{tab:error_expect_inf_category}
shows that the error items have disproportionately higher rates of having mismatch
expected inference category and labels than the correct items.\mcdm{rephrase previous sentence}
Note that there are also a large number of mismatch items that are predicted
correctly by the model in MegaVeridicality and RP.

We found that this is because there are many clause-embedding verbs with
observed labels that are systematically different from the signatures, as we elaborate below.\mcdm{give section, but I think it would be better to say something like: the reverse pattern that we see for MV and RP can be explained by ...}

\begin{table}[t!]
\resizebox{\linewidth}{!}{%
\begin{tabular}{llrrr}
  \toprule
                                  &         & Mismatch \# & Mismatch \% & Total\\
  \midrule
                                   & correct                       & 160                        & 23.8                         & 671                        \\
\multirow{-2}{*}{MegaVeridicality} & \cellcolor[HTML]{F5DED6}error & \cellcolor[HTML]{F5DED6}12 & \cellcolor[HTML]{F5DED6}57.1 & \cellcolor[HTML]{F5DED6}21 \\
                                   & correct                       & 43                         & 8.6                          & 501                        \\
\multirow{-2}{*}{CB}               & \cellcolor[HTML]{F5DED6}error & \cellcolor[HTML]{F5DED6}11 & \cellcolor[HTML]{F5DED6}42.3 & \cellcolor[HTML]{F5DED6}26 \\
                                   & correct                       & 210                        & 23.6                         & 890                        \\
\multirow{-2}{*}{RP}               & \cellcolor[HTML]{F5DED6}error & \cellcolor[HTML]{F5DED6}26 & \cellcolor[HTML]{F5DED6}52.0 & \cellcolor[HTML]{F5DED6}50 \\
  \bottomrule
\end{tabular}
}
\caption{Number of items with mismatching label bin and expected inference category
  (Mismatch \#) and their percentages (Mismatch \%) of the total correct and
  error items for each dataset.}
\label{tab:error_expect_inf_category}
\end{table}


The different ways of assigning expected inference considered here all give the
same results: the model struggles on items where the label cannot be predicted
by the surface patterns.
In the next section, we look at what the surface patterns are and what reasoning
is involved for items that require more than surface patterns.


These two ways of assigning expected inference provide complementary information: the signatures measures how well the
labels match the accounts in formal semantics, while this measures how
in-distribution the test sets are.








\paragraph{CB}
We assign the expected inference category (results shown in
Table~\ref{tab:error_expect_inf_category})in the following way:
  1.\ the neg-raising instances are nonfactual,
  2.\ the factive verbs are factual,
  3.\ polar questions are neutral,
  4.\ modal environment is positive.
As shown in Table~\ref{tab:error_expected_inf_category},
while items with a mismatch between the gold label category and
the expected inference constitutes 10\% of the data with expected inference assigned, they make up 42\% of
the error items.
